Revisiting the Implied Remaining Variance framework of Carr and Sun (2014): Locally consistent dynamics and sandwiched martingales

Implied volatility is at the very core of modern finance, notwithstanding standard option pricing models continue to derive option prices starting from the joint dynamics of the underlying asset price and the spot volatility. These models often cause difficulties: no closed formulas for prices, demanding calibration techniques, unclear maps between spot and implied volatility. Inspired by the practice of using implied volatility as quoting system for option prices, models for the joint dynamics of the underlying asset price and the implied volatility have been proposed to replace standard option pricing models. Starting from Carr and Sun (2014), we develop a framework based on the Implied Remaining Variance where minimal conditions for absence of arbitrage are identified, and smile bubbles are dealt with. The key concepts arising from the new IRV framework are those of locally consistent dynamics and sandwiched martingale. Within the new IRV framework, the results of Schweizer and Wissel (2008b) are reformulated, while those of El Amrani, Jacquier and Martini (2021) are independently derived.

==> Examples/BS.tex <==
\section{Examples}
\label{sec:examples}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Black-Scholes model}

Suppose $\omega$ satisfy the IRV master SDE with $b_t \equiv 0$, $c_t  \equiv 0$, $\sigma_t \equiv \sigma \in (0,+\infty)$ and $\omega_0 = \sigma^2 T$. It corresponds to the IRV model
\[
\begin{cases}
	S_t = S_0 \cdot \exp\Big\{\sigma \, W_t - \frac{\sigma^2}{2} t \Big\}, \qquad S_0 > 0 \\
	\omega_t = \sigma^2 (T-t)
\end{cases}
\]
which is nothing else than the Black-Scholes model with volatility $\sigma$. As one can expect, the dynamics of $\omega$ is globally consistent, ensuring absence of arbitrage.

Being $\partial \omega / \partial K \equiv 0$, it is easy to show the equivalence between globally IRV dynamics and Eq.~(4.18)--(4.19) of~\textcite{SchweizerWissel:2008b}. Indeed, the local implied volatility, $X$, and the price level, $Y$, are in this case equal to
\[
\begin{cases}
	X_t \coloneqq \frac{\varphi \big( \mathcal{N}^{-1} \big( - \frac{\partial C_t(K)}{\partial K}\big) \big)}{\sqrt{T-t} \, K \, \frac{\partial^2 C_t(K)}{\partial K^2}} = \sqrt{\frac{\omega_t}{T-t}}\\
	Y_t  \coloneqq \sqrt{T-t} \cdot \mathcal{N}^{-1} \Big( - \frac{\partial C_t(K_0)}{\partial K}\Big) = d_-\big(k_t^0,\sqrt{\omega_t}\big) \cdot \sqrt{T-t} 
\end{cases}
\]
where $k_t^0 \coloneqq \log(K_0/S_t)$, being $K_0 \in (0,\infty)$ a fixed constant.

Assuming that $\omega$ follows a globally consistent dynamics with $b_t \equiv 0$ and $c_t \equiv 0$, we apply It\^o formula to $Y$:
\[
dY_t = \frac{1}{2} \frac{Y_t}{T-t} \Bigg\{ - \frac{(\omega_t + 2k^0_t) \, \sigma^2 (T-t)}{2 \omega_t Y_t} \sqrt{\frac{T-t}{\omega_t}} - 1 \Bigg\} \, dt + \sigma \sqrt{\frac{T-t}{\omega_t}} \, dW_t.
\]
Defining
\[
\beta_t \coloneqq \frac{1}{2} \frac{Y_t}{T-t} \Bigg\{ - \frac{(\omega_t + 2k^0_t) \, \sigma^2 (T-t)}{2 \omega_t Y_t} \sqrt{\frac{T-t}{\omega_t}} - 1 \Bigg\} \qquad \text{and} \qquad \gamma_t \coloneqq \sigma \sqrt{\frac{T-t}{\omega_t}}, 
\]
we have
\[
\beta_t = \frac{1}{2} \frac{Y_t}{T-t} \Bigg\{ - \frac{(\omega_t + 2k^0_t) \sqrt{T-t}}{2 Y_t\sqrt{\omega_t}} \sigma^2 \frac{T-t}{\omega_t}- 1 \Bigg\} = \frac{1}{2} \frac{Y_t}{T-t} \bigg( \sigma^2 \frac{T-t}{\omega_t} - 1 \bigg) = \frac{1}{2} \frac{Y_t}{T-t} \big(  \gamma_t^2 - 1 \big)
\]
which is exactly Eq.~(4.18) of~\textcite{SchweizerWissel:2008b}.

Applying It\^o formula to $X$, we have
\[
dX_t = \frac{1}{2} \bigg( \frac{1}{T-t} - \frac{\sigma_t^2}{\omega_t} \bigg) X_t \, dt 
\]
that is, according with the notation of~\citeauthor{SchweizerWissel:2008b}, 
\[
u_t = \frac{1}{2} \bigg( \frac{1}{T-t} - \frac{\sigma_t^2}{\omega_t} \bigg) \qquad \text{and} \qquad v_t \equiv 0.
\]
Hence,
\[
u_t = \frac{1}{T-t} \bigg( \frac{1}{2} - \frac{1}{2} \sigma^2 \frac{T-t}{\omega_t} \bigg) = \frac{1}{T-t} \bigg( \frac{1}{2} - \frac{1}{2} \gamma_t^2 \bigg)
\]
which is exactly Eq.~(4.19) of~\textcite{SchweizerWissel:2008b}.

On the other hand,~\citeauthor{SchweizerWissel:2008b} shows that Black-Scholes model satisfies their equations and it implies $X_t = \sigma$. Therefore, we have
\[
d\omega_t = d\big(X_t^2 (T-t)\big) = d\big(\sigma^2 (T-t) \big) = - \sigma^2 \, dt
\]
which is exactly the global consistent dynamics we obtain when $b_t \equiv 0$ and $c_t \equiv 0$ in the IRV master SDE.

Finally, suppose that the underlying asset satisfies the Black-Scholes model with time-dependent volatility, i.e. $\sigma = \sigma(t)$ is a deterministic function of time. It corresponds to the IRV model
\[
\begin{cases}
	S_t = S_0 \cdot \exp\Big\{\int_0^t \sigma(s) \, dW_s - \frac{1}{2} \int_0^t \sigma^2(s) \, ds \Big\}, \qquad S_0 > 0 \\
	\omega_t = \int_t^T \sigma^2(s) \, ds
\end{cases}
\]
that is
\[
\omega_t = \int_0^T \sigma^2(s) \, ds - \int_0^t \sigma^2(s) \, ds.
\]
Therefore, $\omega$ satisfies again the IRV master SDE with $b_t \equiv 0$, $c_t \equiv 0$ and $\omega_0 = \int_0^T \sigma^2(s) \, ds$. Assuming as usual that $\sigma(t) \in (0,+\infty)$ for any $t$, the dynamics of $\omega$ is also globally consistent.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Stochastic Volatility Inspired parametrization}

The main question of~\textcite{ElAmraniJacquierMartini:2020} is whether there exist IRV smile models such that the smiles at any time satisfy the symmetric \emph{Stochastic Volatility Inspired (SVI)} parametrization (see~\cite{Gatheral:2004},~\cite{Gatheral:2006},~\cite{GatheralJacquier:2014}) and the market is arbitrage-free. Their findings are that if such models exist, then they imply always flat IRV smiles. The Black-Scholes model with time-dependent volatility is an example. The aim of this section is to show that the dynamics corresponding to such models are actually globally consistent.

On $\big(\Omega,\mathcal{F},(\mathcal{F}_t)_{t \ge 0},\mathbb{Q}\big)$, consider the collection of strike prices $\{K_i\}_{i \in \mathcal{I}}$ and the IRV smile model
\begin{equation}\label{eq:SVI1}
	\begin{cases}
		S_t = \exp\Big\{\int_0^t \sigma_s \, dW_s - \frac{1}{2} \int_0^t \sigma_s^2 \, ds\Big\} \\
		\omega_{i,t} = \frac{1}{2} \Big( \theta_t + \sqrt{\theta_t^2 + \psi_t^2 k_{i,t}^2}\Big) 
	\end{cases}
\end{equation}
where $W$ is a standard Brownian motion, $\sigma$ is an almost surely positive process satisfying the Novikov condition,\footnote{$\mathbb{E}\Big[\exp \Big\{ \frac{1}{2} \int_0^T \sigma_t^2 \, dt \Big\}\Big] < \infty$} and, according with the SVI parametrization,  $\theta$ is the IRV process corresponding to the time-$t$ at-the-money call. Furthermore, assume that
\begin{equation}\label{eq:SVI2}
	\begin{cases}
		d\theta_t = \frac{(\psi_t -4)(\psi_t + 4)}{16} \sigma_t^2 \, dt - \psi_t \sigma_t \, dZ_t \\
		d\psi_t = \mu_t \, dt + \sqrt{\nu_t} \, dZ_t 
	\end{cases}
\end{equation}
where $Z$ is a standard Brownian motion independent of $W$.

\citeauthor{ElAmraniJacquierMartini:2020} prove that the market described by Eq.~\eqref{eq:SVI1} is arbitrage-free only if Eq.~\eqref{eq:SVI2} is satisfied with $\mu_t \equiv 0$ and $\nu_t \equiv 0$ (i.e., $\psi_t \equiv \psi$), and $\theta_t$ is almost surely finite and converges to $0$ as $t \rightarrow T$. They prove that these conditions also imply that $\psi = 0$ and the smiles are flat at any time.

For notational simplicity, we set 
\[
A_{i,t} \coloneqq \sqrt{\theta_t^2 + \psi_t^2 k_{i,t}^2}
\]
so that
\[
\omega_{i,t} = \frac{1}{2} \big( \theta_t + A_{i,t} \big).
\]

We apply It\^o formula to $\omega_{i}$:
\begin{multline}\label{eq:SVI3}
	d\omega_{i,t} = \frac{1}{2} \Bigg[ \bigg( 1 + \frac{\theta_t}{A_{i,t}}\bigg) \frac{(\psi_t -4)(\psi_t + 4)}{16} + \frac{\psi_t k_{i,t}^2}{A_{i,t}} \frac{\mu_t}{\sigma_t^2} + \frac{\psi_t^2 k_{i,t}}{2 A_{i,t}} \\
	+ \frac{1}{2 A_{i,t}^3} \bigg( \psi_t^4 k_{i,t}^2 + \theta_t^2 k_t^2 \frac{\nu_t}{\sigma_t^2} + \theta_t^2 \psi_t^2 \bigg) + \frac{\theta_t \psi_t^2 k_{i,t}^2}{A_{i,t}^3} \frac{\sqrt{\nu_t}}{\sigma_t} \Bigg] \sigma_t^2 \, dt \\
	+ \frac{1}{2} \Bigg[ \frac{\psi_t k_{i,t}^2}{A_{i,t}} \frac{\sqrt{\nu_t}}{\sigma_t} - \bigg( 1 + \frac{\theta_t}{A_{i,t}} \bigg) \psi_t \Bigg] \sigma_t  \, dZ_t - \frac{\psi_t^2 k_{i,t}}{2 A_{i,t}} \sigma_t \, dW_t.
\end{multline}
We note that the framework is that of a market with an IRV smile driven by only two independent Brownian motions: $W$, the one driving the underlying asset price; and $Z$, common to all strike prices. 

The IRV smile dynamics is locally consistent only if each individual dynamics in Eq.~\eqref{eq:SVI3} satisfy the no-drift condition of Eq.~\eqref{eq:nodrift}:
\begin{multline*}
	\frac{1}{2} \Bigg[ \bigg( 1 + \frac{\theta_t}{A_{i,t}}\bigg) \frac{(\psi_t -4)(\psi_t + 4)}{16} + \frac{\psi_t k_{i,t}^2}{A_{i,t}} \frac{\mu_t}{\sigma_t^2} + \frac{\psi_t^2 k_{i,t}}{2 A_{i,t}} + \frac{1}{2 A_{i,t}^3} \bigg( \psi_t^4 k_{i,t}^2 + \theta_t^2 k_{i,t}^2 \frac{\nu_t}{\sigma_t^2} + \theta_t^2 \psi_t^2 \bigg) + \frac{\theta_t \psi_t^2 k_{i,t}^2}{A_{i,t}^3} \frac{\sqrt{\nu_t}}{\sigma_t} \Bigg] \\
	= \frac{\psi_t^2 \big(A_{i,t} + \theta_t \big) \omega_{i,t}^2 + 4 \psi_t^2 \big(A_{i,t} + \theta_t \big) \omega_{i,t} + 8 \psi_t^2 k_{i,t} \omega_{i,t}^2 - 4 \psi_t^2 k_{i,t}^2 \big(A_{i,t} + \theta_t \big) + 16 \psi_t^2 k_{i,t}^2 \omega_{i,t} - 32 A_{i,t} \omega_{i,t}^2}{32 A_{i,t} \omega_{i,t}^2} \\
	+ \frac{\psi_t^2 k_{i,t}^2 \sqrt{\nu_t} \big(\omega_{i,t}^2 + 4 \omega_{i,t} - 4 k_{i,t}^2 \big) \Big[ k_{i,t}^2 \sqrt{\nu_t} - 2 \big(A_{i,t} + \theta_t \big) \sigma_t\Big]}{64 A_{i,t}^2 \sigma_t^2 \omega_{i,t}^2}
\end{multline*}
that is
\[
\frac{k_{i,t}^2}{2 \sigma_t A_{i,t}} \bigg[ \bigg( \frac{\theta_t}{2} \frac{\sqrt{\nu_t}}{\sigma_t} + \psi_t^2 \bigg) \frac{\theta_t}{A_{i,t}^2} \sqrt{\nu_t} + \psi_t \frac{\mu_t}{\sigma_t} \bigg] = \frac{\psi_t^2 k_{i,t}^2 \sqrt{\nu_t} \big(\omega_{i,t}^2 + 4 \omega_{i,t} - 4 k_{i,t}^2 \big) \Big[ k_{i,t}^2 \sqrt{\nu_t} - 2 \big(A_{i,t} + \theta_t \big) \sigma_t\Big]}{64 A_{i,t}^2 \sigma_t^2 \omega_{i,t}^2}
\]
and thus
\begin{multline}\label{eq:SVI4}
	\mu_t = \, \Bigg\{ \frac{\psi_t k_{i,t}^2}{32 A_{i,t} \big(A_{i,t} + \theta_t\big)^2}	\Big[ \big(A_{i,t} + \theta_t\big)^2 + 8 \big(A_{i,t} + \theta_t\big) - 16 k_{i,t}^2 \Big] - \frac{\theta_t^2}{2 \psi_t A_{i,t}^2}	\Bigg\} \nu_t \\
	- \Bigg\{	\frac{\psi_t}{16 A_{i,t} \big(A_{i,t} + \theta_t\big)} \Big[ \big(A_{i,t} + \theta_t\big)^2 + 8 \big(A_{i,t} + \theta_t\big) - 16 k_{i,t}^2 \Big] + \frac{\theta_t \psi_t}{A_{i,t}^2}	\Bigg\} \sigma_t \sqrt{\nu_t}
\end{multline}
for any $i \in \mathcal{I}$.

If $\mu_t \equiv 0$ and $\nu_t \equiv 0$, Eq.~\eqref{eq:SVI4} is clearly satisfied for any $i \in \mathcal{I}$ and therefore the IRV smile dynamics is locally consistent.\footnote{We are implicitly assuming that the market is free of static arbitrage at time 0.} If $\theta_t$ is also almost surely finite and converges to $0$ as $t \rightarrow T$, we have $\omega_{i,t}= \theta_t$ and $\tau_{i} = \tau^0_i = T$, for any $i \in \mathcal{I}$ and $t \in [0,T)$. Hence, the IRV smile dynamics is globally consistent.


==> Examples/Old_SVI.tex <==
the following dynamic version of the symmetric SSVI parameterisation
\begin{equation}\label{eq:SSVIw}
	\omega_t = \frac{\theta_t}{2} \bigg( 1 + \sqrt{1+\varphi_t^2 k_t^2} \bigg)
\end{equation}
where $\theta_t$, $\varphi_t$ are two stochastic processes and $k_t \equiv \log(K/S_t)$. In particular, $\theta_t$ represents the IRV process corresponding to the at-the-money European call option at time $t$ maturing at $T$.  They finally assume that $\theta_t$ and $\varphi_t$ are diffusion processes given by
\begin{equation}
	\begin{cases}
		d\theta_t = \theta_{1,t} \, dt + \theta_{2,t} \, dZ_t^{\theta}, \quad \theta_0 > 0 \\
		d\varphi_t = \varphi_{1,t} \, dt + \varphi_{2,t} \, dZ_t^{\varphi}, \quad \varphi_0 > 0 \\
		d\langle Z^{\theta}, Z^{\varphi} \rangle_t = \rho \, dt
	\end{cases}
\end{equation}
where $Z^{\theta}$ and $Z^{\varphi}$ are two Brownian motions. The time-dependent coefficients $\theta_1, \theta_2, \varphi_1, \varphi_2$ are left unspecified, and may be stochastic, adapted to the filtration $(\mathcal{F}_t)_{t \in [0,T]}$.

What they demonstrate is that the following conditions are necessary (but not sufficient) for the market to be free of dynamic arbitrage opportunities in $[0,T]$:
\begin{itemize}
	\item (Lemma 3.4. of EJM) $\theta_t$ converges to zero almost surely at time $T$;
	\item (Theorem 3.5. of EJM) it holds:
	\begin{equation}\label{eq:SSVIdthetadphi}
		\begin{cases}
			d\theta_t = \frac{(\theta_t \varphi_t - 4)(\theta_t \varphi_t + 4)}{16} v_t \, dt - \theta_t \varphi_t \sigma_t \, dZ_t \\
			d\varphi_t = \big( 16 + 16 \varphi_t^2 \theta_t - \theta_t^2 \varphi_t^2 \big) \frac{\varphi_t \sigma_t}{16 \theta_t} \, dt + \varphi_t^2 \sigma_t \, dZ_t
		\end{cases}		
	\end{equation}
	where $Z$ is a Brownian motion independent from $W$.
\end{itemize}

At this point, let $\psi_t \equiv \theta_t \varphi_t$ and apply It\^o formula to it. If Eq.\eqref{eq:SSVIdthetadphi} holds, we find immediately that $d\psi_t = 0$, that is $\psi_t \equiv \psi$ constant.\footnote{Actually, $\psi$ depends on $T$, but, since we are working with a fixed $T$, we suppress the argument.} Since in an arbitrage-free market it must be $\theta_T = 0$, it must be also $\psi = 0$. From this, it easily follows:
\begin{proposition}[Prop. 3.6. of EJM]
	If there exists an IRV model able to guarantee absence of arbitrage on $[0,T]$ and $(\theta_t,\varphi_t)$ solves Eq.~\eqref{eq:SSVIdthetadphi}, then, forn any $t \in [0,T]$, $\theta_t = \int_t^T \sigma_s^2 \, ds$, all the smiles (at $t$, maturing at $T$) are flat, and $\int_t^T \sigma^2_s \, ds \in \mathcal{F}_t$.
\end{proposition}

While the Black-Scholes model with deterministic volatility clearly satisfies all these conditions,~\citeauthor{ElAmraniJacquierMartini:2020} show that there are no non-trivial IRV dynamics capable of doing the same.

The question now is whether an IRV dynamics derived from Eq.~\eqref{eq:SSVIw}--\eqref{eq:SSVIdthetadphi} is consistent with our IRV master SDE.

In an arbitrage-free market, we can rewrite Eq.~\eqref{eq:SSVIw} as
\begin{equation}\label{eq:SSVIw2}
	\omega_t = \frac{1}{2} \big( \theta_t + A_t \big)
\end{equation}
where $A_t = \sqrt{\psi^2 k_t^2 + \theta_t^2}$ and $\psi$ constant, and replace Eq.~\eqref{eq:SSVIdthetadphi} with
\begin{equation}
	\begin{cases}
		d\theta_t = \frac{ (\psi - 4) (\psi + 4)}{16} \sigma_t^2 \, dt - \psi \sigma_t \, dZ_t \\
		\theta_T = 0 \\
		d\langle W, Z \rangle_t = 0 \, dt
	\end{cases}.
\end{equation}
Applying It\^o's formula to $\omega_t$, we obtain:
\begin{equation}\label{eq:SSVIdw}
	\begin{split}
		d\omega_t = & \bigg\{ \frac{ \big( \psi - 4 \big) \big( \psi + 4 \big)}{32} \frac{\big( \theta_t + A_t \big)}{A_t} + \frac{\psi^2 k_t}{4 A_t} + \frac{\psi^2}{4 A_t} \bigg\} \sigma_t^2 \, dt - \psi \bigg(\frac{\theta_t}{2 A_t} + \frac{1}{2}\bigg) \sigma_t \, dZ_t - \frac{\psi^2 k_t}{2 A_t} \sigma_t \, dW_t.
	\end{split}
\end{equation}
Comparing the dynamics in Eq.~\eqref{eq:SSVIdw} with Eq.~\eqref{eq:SDE} in our Theorem~\ref{thr:masterSDE}, we recognize that:
\begin{itemize}
	\item $a_t = \frac{ (\psi - 4) (\psi + 4)}{32} \frac{(\theta_t + A_t)}{A_t} + \frac{\psi^2 k_t}{4 A_t} + \frac{\psi^2}{4 A_t}$;
	\item $b_t = - \frac{\psi}{\omega_t} \Big(\frac{\theta_t}{2 A_t} + \frac{1}{2}\Big)$;
	\item $c_t =  - \frac{\psi^2 k_t}{2 \omega_t A_t}$;
\end{itemize}
and therefore the no-drift condition of Eq.~\eqref{eq:nodrift} becomes:
\begin{multline}\label{eq:SSVInodrift}
	\frac{ \big(\psi - 4\big) \big(\psi + 4\big)}{32} \frac{\big(\theta_t + A_t\big)}{A_t} + \frac{\psi^2 k_t}{4 A_t} + \frac{\psi^2}{4 A_t} \\
	=  \frac{\psi^2}{64A_t^2} \Big[ \big(\theta_t + A_t\big)^2 + \psi^2 k_t^2 \Big] + \frac{\psi^2}{16 \omega_t A^2_t} \Big[\big(\theta_t + A_t \big)^2 + \psi^2 k_t^2\Big] + \frac{\psi^2 k_t^2}{4 A_t} \\
	- \bigg[\frac{\psi^2 k_t^2}{16 \omega_t^2 A_t^2} \Big(\big(\theta_t + A_t \big)^2 + \psi^2 k_t^2 \Big) - \frac{\psi^2 k^2_t}{2 \omega_t A_t} + 1 \bigg].
\end{multline}
Recalling that in an arbitrage-free market it must be $\psi = 0$, Eq.~\eqref{eq:SSVInodrift} clearly holds and then we can conclude that an  IRV dynamics derived from a symmetric SSVI satisfies our IRV master SDE.

==> Examples/Old_SW.tex <==
The results of~\textcite{SchweizerWissel:2008b} for a single option market can be easily mapped into the new IRV framework. 

First of all, we recognize that the process $\mathcal{X}$ in~\textcite{SchweizerWissel:2008b} is nothing else than $\omega / (T-t)$, where we omit the argument $(K)$ because fixed. 

Under the risk-neutral probability $\mathbb{Q}$, Eq.~(3.4)--(3.5) of~\textcite{SchweizerWissel:2008b} can be rewritten as
\begin{equation}\label{eq:SW1}
	\begin{cases}
		dS_t = S_t 
		\begin{bmatrix}
			\sigma_{1,t} & 0
		\end{bmatrix}
		\times 
		\begin{bmatrix}
			dW_t \\
			dZ_t
		\end{bmatrix}, \qquad S_0 = s_0 > 0 \\
		d\mathcal{X}_t = u_t \mathcal{X}_t \, dt + \mathcal{X}_t
		\begin{bmatrix}
			v_{1,t} & v_{2,t}
		\end{bmatrix}
		\times 
		\begin{bmatrix}
			dW_t \\
			dZ_t
		\end{bmatrix}, \qquad \mathcal{X}_0 = x_0 > 0
	\end{cases}
\end{equation}
and the drift restriction in Eq.~(3.7) as
\begin{multline}\label{eq:SW2}
	u_t = \frac{1}{T-t} \bigg( 1 - \frac{\sigma_{1,t}^2 + k_t \sigma_{1,t} v_{1,t} + \frac{1}{4} k_t^2 v_{1,t}^2 + \frac{1}{4} k_t^2 v_{2,t}^2}{\mathcal{X}_t} \bigg) \\
	+ \bigg( \frac{(T-t) \mathcal{X}_t}{16} + \frac{1}{4}\bigg) \big( v_{1,t}^2 + v_{2,t}^2\big) - \frac{1}{2}\sigma_{1,t} v_{1,t}
\end{multline}
where $k_t \coloneqq \log(K/S_t)$.

Assuming Eq.~\eqref{eq:SW1}--\eqref{eq:SW2} hold and $\sigma_1 > 0$, we apply It\^o formula to $\mathcal{\omega}$:
\[
\begin{split}
	d\omega_t = & \, -\mathcal{X}_t \, dt + (T-t) \, d\mathcal{X}_t \\
	= & \, \Bigg[ \frac{v_{2,t}^2 / \sigma_{1,t}^2 + v_{1,t}^2 / \sigma_{1,t}^2}{16} \, \omega_t^2 + \frac{v_{2,t}^2 / \sigma_{1,t}^2 + v_{1,t}^2 / \sigma_{1,t}^2 - 2 v_{1,t} / \sigma_{1,t}}{4} \, \omega_t \\
	& - \bigg( \frac{v_{2,t}^2 / \sigma_{1,t}^2 + v_{1,t}^2 / \sigma_{1,t}^2}{4} k_t^2 + \frac{v_{1,t}}{\sigma_{1,t}} k_t + 1 \bigg) \Bigg] \sigma_{1,t}^2 \, dt + v_{2,t} \omega_t \, dZ_t + v_{1,t} \omega_t \, dW_t.
\end{split}
\]
It is clear that $\omega$ follows a locally consistent dynamics with
\begin{equation}\label{eq:SWbc}
	\begin{cases}
		b_t = v_{2,t} / \sigma_{1,t} \\
		c_t = v_{1,t} / \sigma_{1,t},
	\end{cases}
\end{equation}
the drift restriction on $\mathcal{X}$ identified by~\citeauthor{SchweizerWissel:2008b} is equivalent to the no-drift condition on the IRV in Eq.~\eqref{eq:nodrift}, and their Theorem 3.2 is analogous to our Theorem~\ref{thr:masterSDE}.

Therefore, we can restate their Proposition 3.3 as follows:
\begin{proposition}\label{prop:SW33}
	In the framework of Theorem~\ref{thr:masterSDE}, assume that $S$ follows the dynamics in Eq.~\eqref{eq:SW1} and $b$, $c$, $\sigma_1$ are functions of $t$, $S$, $\omega$:
	\[
	b_t = b(t,S_t,\omega_t), \qquad c_t = c(t,S_t,\omega_t), \qquad \sigma_{1,t} = \sigma_1(t,S_t,\omega_t).
	\]
	With $\sigma_1 > 0$ and $t \in [0,T)$, let
	\begin{multline}\label{eq:SW33}
		\begin{bmatrix}
			\sigma_1(t,S_t,\omega_t) \\
			0
		\end{bmatrix} = - \frac{1}{2} k_t \, \sigma_1(t,S_t,\omega_t)
		\begin{bmatrix}
			c(t,S_t,\omega_t) \\
			b(t,S_t,\omega_t)
		\end{bmatrix} \\
		+ \sqrt{\frac{\omega_t}{T-t}} \cdot \bigg( \begin{bmatrix}
			f_1(t,S_t,\omega_t) \\
			f_2(t,S_t,\omega_t)
		\end{bmatrix} + (T-t) \begin{bmatrix}
			g_1(t,S_t,\omega_t) \\
			g_2(t,S_t,\omega_t)
		\end{bmatrix} \bigg)
	\end{multline}
	where $f, \, g, \, \begin{bmatrix}
		b \sigma_1 & c \sigma_1
	\end{bmatrix}: [0,T] \times (0,\infty)^2 \rightarrow \mathbb{R}^2$ are locally Lipschitz\footnote{A function $f : \Theta \times U \rightarrow \mathbb{R}^k$ is said \emph{locally Lipschitz} on $U$ if $f(\cdot,x)$ is bounded for fixed $x \in U$ and if there exists a continuous function $C(\cdot,\cdot)$ on $U^2$ such that
		\[
		\big\lvert f(\theta,x) - f(\theta,x')\big\rvert \le C(x,x') \, \lvert x - x' \rvert, \qquad \forall x, x' \in U, \, \theta \in \Theta.
		\]} on $(0,\infty)^2$ and satisfy
	\begin{equation}\label{eq:SWcon}
		\begin{cases}
			\big\lvert f(t,S_t,\omega_t) \big\rvert = 1 \\
			\big\lvert g(t,S_t,\omega_t)\big\rvert \le const \\
			\sigma_1(t,S_t,\omega_t) \cdot \sqrt{b^2(t,S_t,\omega_t) + c^2(t,S_t,\omega_t)} \le \frac{const}{1 + \sqrt{\omega_t / (T-t)} + \lvert k_t \rvert}
		\end{cases}
	\end{equation}
	where $const$ denotes a generic positive constant whose value can change from one line to the next. Then the IRV master SDE has a unique solution, whose dynamics is globally consistent.
\end{proposition}

\begin{proof}
	According with Eq.~\eqref{eq:SW1}, Eq.~(3.8) of~\textcite{SchweizerWissel:2008b} reads as
	\[
	\begin{bmatrix}
		\sigma_1(t,S_t,\omega_t) \\
		0
	\end{bmatrix} \coloneqq - \frac{1}{2} k_t 
	\begin{bmatrix}
		v_1(t,S_t,\omega_t) \\
		v_2(t,S_t,\omega_t)
	\end{bmatrix}
	+ \sqrt{\frac{\omega_t}{T-t}} \cdot \bigg( \begin{bmatrix}
		f_1(t,S_t,\omega_t) \\
		f_2(t,S_t,\omega_t)
	\end{bmatrix} + (T-t) \begin{bmatrix}
		g_1(t,S_t,\omega_t) \\
		g_2(t,S_t,\omega_t)
	\end{bmatrix} \bigg).
	\]
	Due to Eq.~\eqref{eq:SWbc}, we have immediately Eq.~\eqref{eq:SW33}.
	%	\[
	%	\begin{cases}
	%		\sigma(t,S_t,\omega_t) = - \frac{1}{2} k_t \, c(t,S_t,\omega_t) \, \sigma(t,S_t,\omega_t) + \sqrt{\frac{\omega_t}{T-t}} \cdot \big( f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t) \big) \\
	%		0 = - \frac{1}{2} k_t \, b(t,S_t,\omega_t) \, \sigma(t,S_t,\omega_t) + \sqrt{\frac{\omega_t}{T-t}} \cdot \big( f_2(t,S_t,\omega_t) + (T-t) \, g_2(t,S_t,\omega_t) \big).
	%	\end{cases}
	%	\]
	%	\[
	%	\Longrightarrow \qquad 
	%	\begin{cases}
	%		\sigma(t,S_t,\omega_t) = \frac{2}{2 + k_t \, c(t,S_t,\omega_t)} \sqrt{\frac{\omega_t}{T-t}} \cdot \big( f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t) \big) \\
	%		\sigma(t,S_t,\omega_t) = \frac{2}{k_t \, b(t,S_t,\omega_t)} \sqrt{\frac{\omega_t}{T-t}} \cdot \big( f_2(t,S_t,\omega_t) + (T-t) \, g_2(t,S_t,\omega_t) \big)
	%	\end{cases}
	%	\]
	%	\[
	%	\Longrightarrow \qquad \frac{f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t)}{2 + k_t \, c(t,S_t,\omega_t)} = \frac{f_2(t,S_t,\omega_t) + (T-t) \, g_2(t,S_t,\omega_t)}{k_t \, b(t,S_t,\omega_t)}
	%	\]
	%	\[
	%	\Longrightarrow \qquad b(t,S_t,\omega_t) = \frac{2 + k_t \, c(t,S_t,\omega_t)}{k_t} \cdot \frac{f_2(t,S_t,\omega_t) + (T-t) \, g_2(t,S_t,\omega_t)}{f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t)}.
	%	\]
	Under all the hypotheses, Proposition 3.3 of~\textcite{SchweizerWissel:2008b} ensures that the system in Eq.~\eqref{eq:SW1}--\eqref{eq:SW2} has a unique solution $(S,\mathcal{X})$, which is positive and nonexploding on $[0,T]$. Since that system is equivalent to one with identical $S$ and $\omega \coloneqq \mathcal{X} \, (T-t)$ following a locally consistent dynamics, under the same hypotheses we have that $\omega$ is the unique solution of the IRV master SDE and follows a globally consistent dynamics.
\end{proof}

%\begin{corollary}
%	In Proposition~\ref{prop:SW33}, if it is
%	\[
%	\begin{cases}
%		k_t \ne 0 \\
%		b(t,S_t,\omega_t) \ne 0 \\
%		c(t,S_t,\omega_t) \ne -2 / k_t \\
%		f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t) \ne 0
%	\end{cases}
%	\]
%	then Eq.~\eqref{eq:SW33} reads as
%	\begin{equation}\label{eq:SWb}
%	b(t,S_t,\omega_t) = \frac{2 + k_t \, c(t,S_t,\omega_t)}{k_t} \cdot F(t,S_t,\omega_t)
%	\end{equation}
%	where 
%	\[
%	F(t,S_t,\omega_t) \coloneqq \frac{f_2(t,S_t,\omega_t) + (T-t) \, g_2(t,S_t,\omega_t)}{f_1(t,S_t,\omega_t) + (T-t) \, g_1(t,S_t,\omega_t)}
%	\]
%	and the last constraint in Eq.~\eqref{eq:SWcon} as
%	\begin{multline*}
%		\Big[ 1 + F^2(t,S_t,\omega_t) \Big] c^2(t,S_t,\omega_t) + \frac{4 F^2(t,S_t,\omega_t)}{k_t} c(t,S_t,\omega_t) + \frac{4 F^2(t,S_t,\omega_t)}{k_t^2}  \\
%		\le \frac{const}{\sigma^2(t,S_t,\omega_t) \, \big(1 + \sqrt{\omega_t / (T-t)} + \lvert k_t \rvert\big)^2}.
%	\end{multline*}
%\end{corollary}

\begin{example}
	Let 
	\[
	\begin{cases}
		f_1(t,S_t,\omega_t) \equiv 1 \\
		g_1(t,S_t,\omega_t) \equiv 0 \\
		f_2(t,S_t,\omega_t) = g_2(t,S_t,\omega_t) \equiv 0 \\
		b(t,S_t,\omega_t) \equiv 0 \\
		c(t,S_t,\omega_t) \equiv 0
	\end{cases}
	\]
	and
	\[
	\sigma_1(t,S_t,\omega_t) = \sigma_1(t) = \sigma_{1,t}.
	\]
	Then, we have
	\[
	\sigma_{1,t} = \sqrt{\frac{\omega_t}{T-t}} \qquad \Longleftrightarrow \qquad \omega_t = \sigma^2_{1,t} \, (T-t)
	\]
	which corresponds to the Black-Scholes model with time-dependent volatility.
\end{example}

%\begin{example}
%	Let 
%	\[
%	\begin{cases}
%		f_1(t,S_t,\omega_t) \equiv 1 \\
%		g_1(t,S_t,\omega_t) \equiv 0 \\
%		f_2(t,S_t,\omega_t) = g_2(t,S_t,\omega_t) \equiv 0 \\
%		b(t,S_t,\omega_t) \equiv 0 \\
%		c(t,S_t,\omega_t) = \frac{1}{\sigma_1(t,S_t,\omega_t) \, \big(1 + \sqrt{\omega_t / (T-t)} + \lvert k_t \rvert \big)}
%	\end{cases}
%	\]
%	Then
%	\[
%	\sigma_1(t,S_t,\omega_t) = - \frac{k_t}{2 \big(1 + \sqrt{\omega_t / (T-t)} + \lvert k_t \rvert \big)} + \sqrt{\frac{\omega_t}{T-t}}.
%	\]
%\end{example}

\begin{example}
	Let 
	\[
	\begin{cases}
		f_1(t,S_t,\omega_t) \equiv 1 \\
		g_1(t,S_t,\omega_t) \equiv 0 \\
		f_2(t,S_t,\omega_t) = g_2(t,S_t,\omega_t) \equiv 0 \\
		b(t,S_t,\omega_t) \equiv 0 \\
	\end{cases}
	\]
	From Eq.~\eqref{eq:SW33}, it must be
	\begin{equation}\label{eq:ex1}
		\sigma_1(t,S_t,\omega_t) = - \frac{1}{2} k_t \, \sigma_1(t,S_t,\omega_t) \, c(t,S_t,\omega_t) + \sqrt{\frac{\omega_t}{T-t}}.
	\end{equation}
	
	Assume $k = 0$. Eq.~\eqref{eq:ex1} implies
	\[
	\sigma_1(t,S_t,\omega_t) = \sqrt{\frac{\omega_t}{T-t}},
	\]
	while the last condition of Eq.~\eqref{eq:SWcon} reads as
	\[
	\big\lvert c(t,S_t,\omega_t) \big\rvert \le \frac{const}{ \sqrt{\frac{\omega_t}{T-t}} \, \Big( 1 +  \sqrt{\frac{\omega_t}{T-t}} \Big)}.
	\]
	In particular, we can set
	\[
	\big\lvert c(t,S_t,\omega_t) \big\rvert = \frac{2}{ \sqrt{\frac{\omega_t}{T-t}} \, \Big( 1 +  \sqrt{\frac{\omega_t}{T-t}} \Big)}.
	\]
	
	On the other hand, assume $k \ne 0$ and solve Eq.~\eqref{eq:ex1} w.r.t. $c$. We obtain:
	\begin{equation}\label{eq:exc}
		c(t,S_t,\omega_t) = \frac{2}{k_t \, \sigma_1(t,S_t,\omega_t)} \bigg(\sqrt{\frac{\omega_t}{T-t}} - \sigma_1(t,S_t,\omega_t)\bigg).
	\end{equation}
	Replacing $c$ in the last condition of Eq.~\eqref{eq:SWcon}, we find that it must be
	\[
	\sigma_1(t,S_t,\omega_t) \cdot \bigg\lvert \frac{2}{k_t \, \sigma_1(t,S_t,\omega_t)} \bigg( \sqrt{\frac{\omega_t}{T-t}} - \sigma_1(t,S_t,\omega_t)\bigg)\bigg\rvert \le \frac{const}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert}
	\]
	that is, assuming $const = 2$,
	\[
	\bigg\lvert \sqrt{\frac{\omega_t}{T-t}} - \sigma_1(t,S_t,\omega_t) \bigg\rvert \le \frac{\lvert k_t \rvert}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert}.
	\]
	%	Now, we have to distinguish between two cases:
	%	\begin{itemize}
	%		\item If $\Big\lvert \sqrt{\frac{\omega_t}{T-t}} - \sigma_1(t,S_t,\omega_t) \Big\rvert \ge 0$, then
	%		\[
	%		\sqrt{\frac{\omega_t}{T-t}} - \frac{\lvert k_t \rvert}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert} \le \sigma_1(t,S_t,\omega_t) \le \sqrt{\frac{\omega_t}{T-t}}.
	%		\]
	%		In particular, we can set
	%		\[
	%		\sigma_1(t,S_t,\omega_t) = \sqrt{\frac{\omega_t}{T-t}} - \frac{\lvert k_t \rvert}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert}
	%		\]
	%		so that, replacing this expression for $\sigma_1$ in Eq.~\eqref{eq:exc}, we have
	%		\[
	%		c(t,S_t,\omega_t) = \frac{2}{\sgn(k_t) \, \sqrt{\frac{\omega_t}{T-t}} \, \Big(1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert \Big) - k_t}
	%		\]
	%	\end{itemize}
	If $\Big[ \sqrt{\frac{\omega_t}{T-t}} - \sigma_1(t,S_t,\omega_t) \Big] < 0$, then it must hold
	\[
	\sqrt{\frac{\omega_t}{T-t}} < \sigma_1(t,S_t,\omega_t) \le \sqrt{\frac{\omega_t}{T-t}} + \frac{\lvert k_t \rvert}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert}.
	\]
	In particular, we can set
	\[
	\sigma_1(t,S_t,\omega_t) = \sqrt{\frac{\omega_t}{T-t}} + \frac{\lvert k_t \rvert}{1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert} > \sqrt{\frac{\omega_t}{T-t}} \ge 0
	\]
	so that, replacing $\sigma_1$ in Eq.~\eqref{eq:exc}, we have
	\[
	c(t,S_t,\omega_t) = - \frac{2}{\frac{k_t}{\lvert k_t \rvert} \, \sqrt{\frac{\omega_t}{T-t}} \, \Big(1 + \sqrt{\frac{\omega_t}{T-t}} + \lvert k_t \rvert \Big) + k_t}.
	\]
\end{example}

Proposition~\ref{prop:SW33} is relevant because it ensures the existence of globally consistent dynamics. However, it prescribes an expression for the spot volatility. This contrasts with the aim of the new framework: an IRV model for arbitrage-free markets, leaving the spot volatility dynamics unspecified.

==> Sandwiched_martingales/Sandwiched_martingales_Computations.tex <==
%\begin{gather*}
%BS: \mathbb{R}^2 \rightarrow \mathbb{R}^2 \\
%(k,v) \mapsto (k,c)
%\end{gather*}

%\begin{gather*}
%	BS(k,v) = 
%	\begin{bmatrix}
%		k \\
%		\mathcal{N}(d_+) - e^k \mathcal{N}(d_-)
%	\end{bmatrix}
%\end{gather*}

%\begin{gather*}
%	BS^{\leftarrow}: \mathbb{R}^2 \rightarrow \mathbb{R}^2 \\
%	(k,c) \mapsto (k,v)
%\end{gather*}

%\[
%J = 
%\begin{bmatrix}
%	1 & 0 \\
%	\frac{\partial \mathcal{N}(d_+) - e^k \mathcal{N}(d_-)}{\partial k} & \frac{\partial \mathcal{N}(d_+) - e^k \mathcal{N}(d_-)}{\partial v}
%\end{bmatrix}
%\]

%\[
%d_+ = - \frac{k}{v} + \frac{v}{2} \qquad d_- = d_+ - v
%\]

%\[
%\frac{\partial d_+}{\partial v} =  \frac{k}{v^2} + \frac{1}{2} \qquad \frac{\partial d_-}{\partial v} =  \frac{k}{v^2} - \frac{1}{2}
%\]

%\[
%\begin{split}
%	\frac{\partial \mathcal{N}(d_+) - e^k \mathcal{N}(d_-)}{\partial v} & = \varphi(d_+) \bigg( \frac{k}{v^2} + \frac{1}{2} \bigg) - e^k \varphi(d_-) \bigg( \frac{k}{v^2} - \frac{1}{2} \bigg) \\
%	& = \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}}\bigg( \frac{k}{v^2} + \frac{1}{2} \bigg) - e^k \frac{e^{-\frac{d_-^2}{2}}}{\sqrt{2\pi}}\bigg( \frac{k}{v^2} - \frac{1}{2} \bigg) \\
%	& = \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}} \bigg[ \bigg( \frac{k}{v^2} + \frac{1}{2} \bigg) - e^k e^{-\frac{d_-^2 - d_+^2}{2}} \bigg( \frac{k}{v^2} - \frac{1}{2} \bigg) \bigg] \\
%	& = \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}} \bigg[ \bigg( \frac{k}{v^2} + \frac{1}{2} \bigg) - \bigg( \frac{k}{v^2} - \frac{1}{2} \bigg) \bigg] \\
%	& = \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}} 
%\end{split}
%\]

%\[
%J = 
%\begin{bmatrix}
%	1 & 0 \\
%	\frac{\partial \mathcal{N}(d_+) - e^k \mathcal{N}(d_-)}{\partial k} & \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}} 
%\end{bmatrix}
%\]

%\[
%\lvert J \rvert = \det 
%\begin{bmatrix}
%	1 & 0 \\
%	\frac{\partial \mathcal{N}(d_+) - e^k \mathcal{N}(d_-)}{\partial k} & \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}} 
%\end{bmatrix}
%= - \frac{e^{-\frac{d_+^2}{2}}}{\sqrt{2\pi}}  \neq 0 
%\]

==> Sandwiched_martingales/Sandwiched_martingales_v1.tex <==
\subsection{Version 1}

With abuse of notation, we denote with $BS^{\leftarrow}$ the function
\begin{gather*}
	BS^{\leftarrow} : \mathbb{R} \times [0,+\infty) \rightarrow [0,+\infty] \\
	(k,c) \mapsto v
\end{gather*}
where $v$ is such that
\[
c = BS\big(k,v\big).
\]

\begin{remark}
	\textit{IS $BS^{\leftarrow}$ WELL DEFINED? IS IT A FUNCTION? $BS^{\leftarrow} \in \mathcal{C}^2$?}
\end{remark}

\begin{theorem}\label{thr:sandwiched}
	Let $\big(\Omega, \mathcal{F}, (\mathcal{F}_t)_{t \ge 0},\mathbb{Q}\big)$ be a filtered probability space accommodating two independent Brownian motions $W$ and $Z$, and an almost surely positive and finite random variable $S_0$, independent of $\mathcal{F}^W_{\infty}$ and $\mathcal{F}^Z_{\infty}$, and with known distribution. Let $(\mathcal{F}_t)_{t \ge 0}$ be the augmented filtration defined as in Theorem~\ref{thr:masterSDE}.
	
	Furthermore:
	\begin{itemize}
		\item $\sigma \in L^2_{loc}\big((0,+\infty)\big)$ is such that the process $S$, satisfying 
		\[
		S_t = S_0 \cdot \exp\bigg\{ \int_0^t \sigma_s \, dW_s - \frac{1}{2} \int_0^t \sigma_s^2 \, ds \bigg\}, \qquad a.s.
		\]
		for any $t \in [0,+\infty)$, is a martingale. 
		\item $C$ is a progressively measurable process with continuous paths and such that
		\[
		\begin{cases}
			(S_0-K)_+ < C_0 < S_0 \\
			(S_t-K)_+ \le C_t \le S_t
		\end{cases} \qquad a.s.
		\]
		\item For $n \ge 1$, define the following sequences of stopping times
		\[
		\tau_n^0 \coloneqq \inf \bigg\{t > 0: C_t \le (S_t-K)_+ + \frac{1}{n} \bigg\} \qquad \text{and} \qquad \tau_n^{\infty} \coloneqq \inf \bigg\{t > 0: C_t \ge S_t - \frac{1}{n} \bigg\}
		\]
		and set $\tau_n \coloneqq \tau^0_n \wedge \tau_n^{\infty}$.
	\end{itemize}
	
	Then the process $C^{\tau_n}$ is a martingale and $\langle C^{\tau_n} \rangle$ is an almost surely absolutely continuous function of time if and only if the process 
	\[
	\omega^{\tau_n}_t \coloneqq \Big( {BS}^{\leftarrow} \big(k^{\tau_n}_t, C^{\tau_n}_t / S_t^{\tau_n}\big)\Big)^2
	\]
	where $k_t \coloneqq \log(K/S_t)$ and $n \ge 1$, follows a locally consistent dynamics.
\end{theorem}

\begin{proof}
	For $n \ge 1$, let $C^{\tau_n}$ be a martingale and $\langle C^{\tau_n} \rangle$ an almost surely absolutely continuous function of time. By the martingale representation theorem, there exist two measurable adapted processes $\nu$ and $\lambda$ such that 
	\[
	\int_0^{t \wedge \tau_n} \big( \nu_s^2 + \lambda^2_s \big) \, ds < \infty, \qquad a.s.
	\]
	and
	\[
	C^{\tau_n}_t = C_0 + \int_0^{t \wedge \tau_n} \nu_s \, dW_s + \int_0^{t \wedge \tau_n} \lambda_s \, dZ_s, \qquad a.s. \\
	\]
	By definition of $\omega^{\tau_n}$, we have 
	\[
	C^{\tau_n}_t = S_t^{\tau_n} \cdot BS\bigg(k_t^{\tau_n},\sqrt{\omega^{\tau_n}_t}\bigg).
	\]
	Being $BS$ a strictly increasing function w.r.t. $\sqrt{\omega^{\tau_n}}$, it is almost surely $\omega^{\tau_n} \in (0,+\infty)$. Then
	\[
	C_t^{\tau_n} = S_t^{\tau_n} \cdot \mathcal{N}\bigg(d_+ \bigg( k^{\tau_n}_t, \sqrt{\omega^{\tau_n}_t}\bigg)\bigg) - K \cdot \mathcal{N}\bigg(d_- \bigg( k^{\tau_n}_t, \sqrt{\omega^{\tau_n}_t}\bigg)\bigg).
	\]
	Since $\omega^{\tau_n}$ is defined as a sufficiently smooth function of $k^{\tau_n}$ and $C^{\tau_n}/S^{\tau_n}$, both driven by $W$ and $Z$, we can apply It\^o formula and write
	\[
	\omega^{\tau_n}_t = \omega_0 + \int_0^{t \wedge \tau_n} \alpha_s \, ds + \int_0^{t \wedge \tau_n} \beta_s \, dZ_s + \int_0^{t \wedge \tau_n} \gamma_s \, dW_s, \qquad a.s.
	\] 
	for some processes $\alpha$, $\beta$ and $\gamma$ such that 
	\[
	\int_0^{t \wedge \tau_n} \big( \alpha_s^2 + \beta^2_s + \gamma_s^2 \big) \, ds < \infty, \qquad a.s.
	\]
	We apply It\^o formula to $C^{\tau_n}$:
	\begin{multline*}
		C^{\tau_n}_t 	= C_0 + \int_0^{t \wedge \tau_n} \bigg( \frac{\partial BS_s}{\partial \omega} \alpha_s + \frac{1}{2} \frac{\partial^2 BS_s}{\partial S^2} S_s^2 \sigma_s^2 + \frac{1}{2} \frac{\partial^2 BS_s}{\partial \omega^2} \big(\beta^2_s + \gamma^2_s \big) + \frac{\partial^2 BS_s}{\partial S \, \partial \omega} \gamma_t S_s \sigma_s \bigg) \, ds \\
		+ \int_0^{t \wedge \tau_n} \bigg( \frac{\partial BS_s}{\partial S} S_s \sigma_s + \frac{\partial BS_s}{\partial \omega} \gamma_s \bigg) \, dW_s + \int_0^{t \wedge \tau} \frac{\partial BS_s}{\partial \omega} \beta_s \, dZ_s, \qquad a.s.
	\end{multline*}
	Since $C^{\tau_n}$ is assumed to be a martingale, it must be
	\[
	\frac{\partial BS_t}{\partial \omega} \alpha_t + \frac{1}{2} \frac{\partial^2 BS_t}{\partial S^2} S_t^2 \sigma_t^2 + \frac{1}{2} \frac{\partial^2 BS_t}{\partial \omega^2} \big(\beta^2_t + \gamma^2_t \big) + \frac{\partial^2 BS_t}{\partial S \, \partial \omega} \gamma_t S_t \sigma_s = 0
	\]
	that is
	\[
	\begin{split}
		\alpha_t & = - \bigg\{ \frac{1}{2} \frac{\partial^2 BS_t}{\partial S^2} \bigg/ \frac{\partial BS_t}{\partial \omega} S_t^2 \sigma_t^2 + \frac{1}{2} \frac{\partial^2 CBS_t}{\partial \omega^2} \bigg/ \frac{\partial BS_t}{\partial \omega} \big(\beta^2_t + \gamma^2_t \big) + \frac{\partial^2 BS_t}{\partial S \, \partial \omega} \bigg/ \frac{\partial BS_t}{\partial \omega} \gamma_t S_t \sigma_t \bigg\} \\
		& = - \bigg\{ \sigma_t^2 + \frac{1}{4} \bigg(\frac{k_t^2}{\omega_t^2} - \frac{1}{\omega_t} - \frac{1}{4} \bigg) \big(\beta^2_t + \gamma^2_t\big) + \bigg( \frac{k_t}{\omega_t} + \frac{1}{2} \bigg) \gamma_t \sigma_t \bigg\}
	\end{split}
	\]
	for any $t \in [0,\tau_n]$. Setting
	\[
	\begin{cases}
		\alpha_t = a_t \sigma_t^2 \\
		\beta_t = b_t \omega_t \sigma_t \\
		\gamma_t = c_t \omega_t \sigma_t
	\end{cases}
	\]
	we have
	\[
	\begin{split}
		a_t \sigma_t^2 & = - \bigg\{ \sigma_t^2 + \frac{1}{4} \bigg(\frac{k_t^2}{\omega_t^2} - \frac{1}{\omega_t} - \frac{1}{4} \bigg) \big(b_t^2 \omega_t^2 \sigma_t^2 + c_t^2 \omega_t^2 \sigma_t^2 \big) + \bigg( \frac{k_t}{\omega_t} + \frac{1}{2} \bigg) c_t \omega_t \sigma_t^2 \bigg\}
	\end{split}
	\]
	that is
	\[
	a_t = \frac{b_t^2 + c_t^2}{16} \omega_t^2 + \frac{b_t^2 + c_t^2 - 2c_t}{4} \omega_t - \bigg( \frac{b_t^2 + c_t^2}{4} k_t^2 + c_t k_t + 1 \bigg), \qquad a.s.
	\]
	for any $t \in[0,\tau_n]$, which is exactly the no-drift condition in Eq.~\eqref{eq:nodrift}. Hence, $\omega^{\tau_n}$ follows a locally consistent dynamics.
	
	On the other hand, if $\omega^{\tau_n}$ follows a locally consistent dynamics, then $C^{\tau_n} \coloneqq S^{\tau_n} \cdot BS\big(k^{\tau_n},\sqrt{\omega^{\tau_n}}\big)$ is a martingale by Theorem~\ref{thr:masterSDE} and
	\[
	\langle C^{\tau_n} \rangle_t = \int_0^{t \wedge \tau_n} \bigg[ \bigg(\frac{K b_s \sqrt{\omega_s} \sigma_s \, \varphi(d_-)}{2}\bigg)^2 + \bigg( S_s \, \mathcal{N}(d_+) + \frac{ K  c_s \sqrt{\omega_s} \, \varphi(d_-)}{2} \bigg)^2 \bigg] \, ds, \qquad a.s.
	\]
	that is $\langle C^{\tau_n} \rangle$ is an a.s. absolutely continuous function of time.
\end{proof}

\begin{example} \label{ex:single}
	Assume that the filtered probability space $\big(\Omega,\mathcal{F},(\mathcal{F}_t)_{t \ge 0},\mathbb{Q}\big)$ describes a market composed by an asset, whose price dynamics is given by
	\[
	\begin{cases}
		dS_t = \sigma_t S_t \, dW_t \\
		S_0 > 0
	\end{cases}
	\]
	where $W$ is a standard Brownian motion and the positive process $\sigma_t$ satisfies the Novikov condition, and by a European call option written on this asset, with strike price $K > 0$ and maturity $T > 0$. Consider a localized situation until $\tau$, where $\tau < T$ is a stopping time and trading can occur only on $[0,\tau] \cup \{T\}$. Such a market is arbitrage-free on $[0,\tau] \cup \{T\}$ if $C^{\tau}$ is a sandwiched martingale, that is if:
	\begin{itemize}
		\item $C^{\tau}$ is a martingale;
		\item $C^{\tau}_t \in \Big(\big(S_t - K \big)_+, S_t \Big)$, for any $t$.
	\end{itemize} 
	Let $N_t$ be a positive martingale independent of $W$ and bounded by 1 on $[0,T]$, for example
	\[
	N_t \coloneqq M_t \cdot \exp\big(-T\big)
	\]
	where $M_t \coloneqq \exp \Big\{ -(Z_t^2-t) - 2 \int_0^t Z_u^2 du \Big\}$ and $Z$ is a Brownian motion independent of $W$. In particular, $N_0 \in (0,1)$. Furthermore, assume $S_0 \ne K$ and define
	\[
	\tau \coloneqq \inf \Big\{ t \in (0,T): S_t = K \Big\}.
	\]
	Then, it is immediate to prove that an explicit example of sandwiched martingale consistent with the no-arbitrage constraints is given by the following stopped process:
	\begin{equation}\label{eq:sanC}
		C^{\tau}_t \coloneqq \big(S_{t \wedge \tau} -K\big)_+ + N_{t \wedge \tau} \cdot  \Big[S_{t \wedge \tau} - \big(S_{t \wedge \tau}-K\big)_+ \Big].
	\end{equation}
	Therefore, by Theorem~\ref{thr:sandwiched}, we know that the IRV process corresponding to the process $C^{\tau}$ in Eq.~\eqref{eq:sanC} is well-defined and its dynamics is described by Eq.~\eqref{eq:sanSDE}--\eqref{eq:sana}. In other words, the IRV process corresponding to $C^{\tau}$ is a solution of the SDE of Eq.~\eqref{eq:sanSDE}--\eqref{eq:sana}.  Continuing the comparison with Theorem~\ref{thr:masterSDE}, the latter allows us to state instead that an IRV dynamics consistent with our IRV master SDE (Eq.~\eqref{eq:SDE}--\eqref{eq:nodrift}) corresponds to a call price process which is a sandwiched martingale, of which Eq.~\eqref{eq:sanC} is an example corresponding to particular choices for the processes $a_t$, $b_t$ and $c_t$. \qedsymbol
\end{example}

It is noteworthy that, in an arbitrage-free market, the price process of a call option with strike $L < K$ is again a sandwiched martingale with values in the range 
\[
\big( [S_{t \wedge \tau} - L]_+, S_{t \wedge \tau} \big) \subset \big( [S_{t \wedge \tau} - K]_+, S_{t \wedge \tau} \big).
\]
Therefore, the  call price process in Eq.~\eqref{eq:sanC} is associated with the price dynamics of all the call options with strike price smaller than $K$. In other words, there is no way to distinguish between the price dynamics of two call options with different strike prices if the call option prices lie always above $[S_{t \wedge \tau}-L]_+$, where $L$ is the smaller strike price.
